Generating Functions for Probabilistic Programs

This paper investigates the usage of generating functions (GFs) encoding measures over the program variables for reasoning about discrete probabilistic programs. To that end, we define a denotational GF-transformer semantics for probabilistic while-programs, and show that it instantiates Kozen's seminal distribution transformer semantics. We then study the effective usage of GFs for program analysis. We show that finitely expressible GFs enable checking super-invariants by means of computer algebra tools, and that they can be used to determine termination probabilities. The paper concludes by characterizing a class of -- possibly infinite-state -- programs whose semantics is a rational GF encoding a discrete phase-type distribution.

==> Programs/dueling_cowboys.tex <==
$\while$ ($\codify{x < 1 and t < 2}$){
	$\pif$ ($\codify{t = 0}$){
		{$\ASSIGN{\codify{x}}{1}$} [a] {$\ASSIGN{\codify{t}}{1}$}$\fatsemi$ $\ASSIGN{\codify{c}}{\codify{c + 1}}$
	} $\pelse$ {
		{$\ASSIGN{\codify{x}}{1}$} [b] {$\ASSIGN{\codify{t}}{0}$}$\fatsemi$ $\ASSIGN{\codify{d}}{\codify{d + 1}}$
	}
}

==> Programs/exp_pgf.tex <==
while(z > 0){
	{z := 0} [$\sfrac{1}{2}$] {z := 1};
	x := x + 1
}
while (x > 0){
	 {x:= x - 1} [$\sfrac{1}{x}$] {abort};
	 c := c + 1
}

==> Programs/geometric.tex <==
$\while$ ($\codify{x = 1}$){
	{$\ASSIGN{\codify{x}}{\codify{0}}$} [$\sfrac{1}{2}$] {$\ASSIGN{\codify{x}}{\codify{1}}$}$\fatsemi$
	$\ASSIGN{\codify{c}}{\codify{c + 1}}$
}

==> Programs/non-termination.tex <==
$\while$ ($\codify{x > 0}$){
	{$\ASSIGN{\codify{x}}{\codify{x - 1}}$} [$\sfrac{1}{\codify{x}}$] {$\ASSIGN{\codify{x}}{\codify{x + 1}}$}
}

==> Programs/random_walk.tex <==
$\while$ ($\codify{x > 0}$){
	{$\ASSIGN{\codify{x}}{\codify{x + 1}}$} [$\sfrac{1}{2}$] {$\ASSIGN{\codify{x}}{\codify{x - 1}}$}$\fatsemi$
	$\ASSIGN{\codify{c}}{\codify{c + 1}}$
}

==> Programs/spline.tex <==
$\while$ ($\codify{x > 0}$){
	{$\ASSIGN{\codify{x}}{\codify{0}}$} [$\sfrac{1}{x}$] {$\ASSIGN{\codify{x}}{\codify{x + 1}}$}$\fatsemi$
	$\ASSIGN{\codiy{c}}{\codify{c + 1}}$
}

==> Sections/closed-forms.tex <==
Precise definition of the term \emph{closed-form}\\(maybe we can use the one from \href{https://www.math.leidenuniv.nl/scripties/SudanBachelor.pdf}{\nolinkurl{leidenuniv.nl}}?)
\begin{lemma}[Operations on Closed Forms]%
	Let \codify{x,y,z} be program variables and \codify{c}, \codify{m} be arbitrary, but fixed natural numbers. Let $G \in \pgf$ be in closed form. Then:
	\begin{itemize}
		\item $\sem{\codify{x := y + z}}(G)$ and $\sem{\codify{x := y + c}}(G)$
		\item $\sem{\codify{x := y} \cdot \codify{c}}(G)$
		\item $\sem{\codify{x := y - c}}(G)$
		\item $\sem{\codify{x} \leq \codify{c}}(G)$
		\item $\sem{\codify{x}\; \equiv_{\codify{m}} \codify{c}}(G)$
	\end{itemize}
can be evaluated on the closed form, i.e., without expanding $G$ into the respective power series representation.
\end{lemma}
\begin{proof}
\end{proof}
\begin{lemma}[Boolean Closure]\label{lem:boolean_closure}
	Let \codify{B} and \codify{B'} be boolean expression in \pgcl, which can be evaluated on closed forms. Then:
	\begin{itemize}
		\item $\sem{\codify{B} \wedge \codify{B'}}(G)$
		\item $\sem{\codify{B} \vee \codify{B'}}(G)$
		\item $\sem{\neg\codify{B}}(G)$
	\end{itemize}
can be evaluated on the closed form, i.e., without expanding $G$ into the respective power series representation.
\end{lemma}
\begin{proof}
	See Appendix \ref{proof:boolean_closure}
\end{proof}


==> Sections/equations.tex <==
% !TEX root = ../samplepaper.tex


In this section, we give semantic and syntactic characterizations of subclasses of $\pgcl$-programs (with loops) whose PGF semantics on every program state is guaranteed to be a rational function, i.e.\ a fraction of two polynomials with real coefficients, which is the solution of an effectively constructable system of linear equations.


\begin{example}
	We reconsider \Pref{prog:geometric} to illustrate the main idea of the approach.
	Closer examination of the program yields that $\sem{W}(CX) = C\cdot\sem{W}(X)$. In this example, this is because the guard $\codify{x = 1}$ does not depend on $\codify{c}$ and the loop body merely increments $\codify{c}$ by 1. Thus following \cref{ex:approx_geo}, we have the \emph{linear} equation
	\begin{align*}
		\sem{W}(X) \eeq \tfrac{1}{2}C \pplus \tfrac{1}{2} C \cdot\sem{W}(X)
	\end{align*}
	with \emph{polynomial coefficients} in $\R[C]$.
	This equation is easily solved with standard arithmetic, the unique solution is the \emph{rational function} $\sem{W}(X) = \tfrac{C}{2-C}$, cf.~\cref{ex:approx_geo}.\hfill$\triangle$
\end{example}


\subsection{Homogeneous-bounded Loops}
\label{ssec:semantic_eqs}	

We now consider a loop $W = \WHILEDO{B}{P}$
and we are interested in the PGF $\sem{W}(\bvec{X}^\sigma)$ for any given input state $\sigma \in \N^k$. 
In this whole~\cref{sec:eqs}, we do not consider overapproximations and thus operate within $\pgf$ only.
The following two conditions are key to our approach:%
%
%
\begin{definition}[Homogeneous and Bounded Variables]
	\label{def:bounded_variables}
	Let $P \in \pgcl{}$ be a program, $B$ be a guard and $\codify{x}_i$ be a program variable. Then:
	\begin{itemize}
		\item $\codify{x}_i$ is called \emph{homogeneous} for $P$ if $\sem{P}(X_i \cdot G) = X_i \cdot \sem{P}(G)$ holds for all $G \in \pgf$.
		\item $\codify{x}_i$ is called \emph{bounded} by $B$ if the set $\{ \sigma_i \mid \sigma \in \N^k \text{ and } \sigma \in B \}$ is finite.
	\end{itemize}%
\end{definition}%
%
%
For example, in \Pref{prog:geometric} the variable $\codify{c}$ is homogeneous for the loop body and the variable $\codify{x}$ is bounded by the loop guard. This motivates the following definition:
%
%
\begin{definition}[Homogeneous-bounded Loops]
	\label{def:hom_bounded_loop}
	The loop $W = \WHILEDO{B}{P}$ is called \emph{homogeneous-bounded (HB)} if the following two conditions hold:
	\begin{enumerate}
		\item For all program variables $\codify{x}$ it either holds that
		\begin{itemize}
			\item $\codify{x}$ is homogeneous for the loop-body $P$ and the guard $B$ is independent of $\codify{x}$, or that
			\item $\codify{x}$ is bounded by the guard $B$.
		\end{itemize}
		\item For all program states $\sigma$ such that $\sigma \models B$ it holds that $\sem{P}(\bvec{X}^\sigma)$ is a polynomial.
	\end{enumerate}%
\end{definition}%
%
%
Notice that the second condition of \cref{def:hom_bounded_loop} is automatically fulfilled whenever $P$ is loop-free because a loop-free program certainly terminates after a finite number of steps and thus can never generate distributions with infinite support.
Hence our example \Pref{prog:geometric} is an HB loop. The bounded random walk (\Pref{prog:random_walk} in \cref{sec:overapprox}) is \emph{not} HB as the variable~$\codify{x}$~is neither bounded by the guard $\codify{x > 0}$ nor is the guard independent of $\codify{x}$. Consequently, HB loops are a proper subclass of \pgcl loops.

In the following we let $\bvec{X}_H$ be the homogeneous and $\bvec{X}_B$ be the bounded variables in an HB loop. Further we write $S_B = \{\sigma \in \N^{|\bvec{X}_B|}\mid \sigma \models B\} = \{\sigma_\ell,\ldots,\sigma_\ell\}$, that is we fix some order on $S_B$. Notice that $S_B$ is indeed finite due to the boundedness of the variables $\bvec{X}_B$.%
%
%
\begin{lemma}[The Equation System]
	\label{lem:rational_loop_equation}
	Let $W = \WHILEDO{B}{P}$ be an HB loop. Let $\sigma_i \in S_B$ be a program state and let $p_i \eeq \sem{P}(\bvec{X}_B^{\sigma_i}) \iin \R[\bvec{X}_H][\bvec{X}_B]$, i.e.\ we write $p_i$ as a polynomial with variables in $\bvec{X}_B$ and coefficients in $\R[\bvec{X}_H]$. Then%
	%
	\begin{align*}
		\sem{W}(\bvec{X}_B^{\sigma_i}) \eeq \sum_{\sigma_j \in S_B} [\bvec{X}_B^{\sigma_j}]_{p_i} \cdot \sem{W}(\bvec{X}_B^{\sigma_j}) \pplus \sum_{\sigma \notin S_B} [\bvec{X}_B^{\sigma}]_{p_i}~.
	\end{align*}%
\end{lemma}%
%
%
Defining the matrix $\bvec{A}_{i,j} = [\bvec{X}_B^{\sigma_j}]_{p_i} \in \R[\bvec{X}_H]^{l \times l}$ and the vector $\bvec{b}_i = \sum_{\sigma \notin S_B} [\bvec{X}_B^{\sigma}]_{p_i} \in \R[\bvec{X}_H]^{l}$ (notice that the entries of these objects are polynomials) for all $i,j=1,\ldots,l$, we can reformulate \cref{lem:rational_loop_equation} in matrix-vector notation:%
%
\begin{align*}
	\label{eq:eqs}
	\tag{$\mathit{EQS}$}
	\bvec{y} \eeq \bvec{A} \bvec{y} \pplus \bvec{b}
\end{align*}%
%
and the vector $\omega = (\sem{W}(\bvec{X}_B^{\sigma_\ell}),\ldots,\sem{W}(\bvec{X}_B^{\sigma_\ell}))$ is a solution of the linear equation system~\eqref{eq:eqs}.
Notice that formally, $\omega \in \pgf^\ell$ is a vector with PGFs as entries. However, we can extend $\omega$ to a linear PGF \emph{transformer} --- an element of type $\bar{\omega} \colon \pgf \to \pgf$ --- in a canonical way: We require that (1) all variables $\bvec{X}_H$ are homogeneous for $\bar{\omega}$, (2) the extension $\bar{\omega}$ behaves like $\omega$ on all states $\sigma_i \in S_B$, i.e.\ $\bar{\omega}(\bvec{X}_B^{\sigma_i}) = \omega_i$ and (3) $\bar{\omega}$ is the identity function on the remaining states $\bvec{X}_B^{\sigma}$, $\sigma \notin S_B$. See \cref{app:equations_first_sec} for the full formal definition of $\bar{\omega}$.
With this definition it is clear that the canonical extension of $\omega$ to the PGF-transformer $\bar{\omega} \colon \pgf \to \pgf$ is $\lfp \Phi_{B,P}$, or in other words, $\sem{W} = \bar{\omega}$.
We also have the following:

\begin{lemma}
	\label{lem:omega_least_sol}
	$\omega$ is the unique least solution of \eqref{eq:eqs} in the domain $\pgf^\ell$.
\end{lemma}
We can now state our main result of this section:%
%
%
\begin{theorem}[HB Loops Preserve Rational PGFs]
	\label{thm:rat_func_semantics}
	Let $W = \WHILEDO{B}{P}$ be an HB loop. Then the vector $\bvec{\omega} = (\sem{W}(\bvec{X}_B^{\sigma_\ell}),\ldots,\sem{W}(\bvec{X}_B^{\sigma_\ell}))$ is the \emph{unique} solution
	of the linear equation system \eqref{eq:eqs} under the additional restriction that
	\begin{align*}
		\label{eq:restric}
		\tag{$\star$}
		\bvec{y}_i = 0 \quad \text{if} \quad \sem{W}(\bvec{X}_B^{\sigma_i}) = 0 \quad \forall \sigma_i \in S_B~.
	\end{align*}
 	Moreover, the PGF $\sem{W}(G)$ is a rational function in $\bvec{X}$ for all input PGFs $G$ that are themselves rational functions in $\bvec{X}$.
\end{theorem}
\begin{proof}[Proof sketch]
	By substituting all variables in the polynomial coefficients of $\bvec{A}$ and $\bvec{b}$ by the constant $1$ in the equation system \eqref{eq:eqs}, we obtain a system that can be interpreted as a finite-state Markov chain $M$.
	Intuitively, this substitution corresponds to abstracting away from all homogeneous variables $\bvec{X}_H$.
	The states of $M$ are the elements $S_B \cup \{\top, \bot\}$ where $\top$ is an additional target and $\bot$ a sink.
	The reachability probabilities with respect to a special target state $\top$ in the Markov chain $M$ are equal to the probability of termination of $W$ under input $\sigma \in S_B$. It is known (e.g.\ \cite{BK08}, Chap.\ 10) that explicitly setting the variables corresponding to states that cannot reach $\top$ in $M$ to zero ensures that the associated equation system has a \textit{unique} solution. We use this fact to show that our system $(EQS)$ together with condition \eqref{eq:restric} then also has a unique solution which is a rational function by Cramer's rule. This then further implies that $\sem{W}(G)$ is always a rational function provided that $G$ itself is. More details are given in \cref{app:equations_first_sec}.
\end{proof}%

\subsection{Sufficient Syntactic Conditions and Example}
\label{ssec:syntactic_eqs}

We already argued that the variable $\codify{c}$ in \Pref{prog:geometric} is homogeneous for the loop body. Indeed, we can prove that \enquote{counter-variables} are homogeneous in general:

\begin{proposition}[Counter-variables are Homogeneous]
	\label{prop:syntactic}
	Let $P$ be a loop-free \pgcl-program such that the program variable $\codify{c}$ exclusively occurs in assignment statements of the form $\codify{c := c + } E$ where $E$ is an arithmetic expression in which $\codify{c}$ does not occur and that never evaluates to a negative number. Then $\codify{c}$ is homogeneous for $P$.
\end{proposition}%
%
%
We conclude the section with a final example.%
%
%
\begin{example}[Dueling Cowboys Example] \Pref{prog:dueling_cowboys} models two dueling cowboys~\cite{DBLP:series/mcs/McIverM05}. The hit rate of the first cowboy is $a$ percent and the hit rate of second cowboy is $b$ percent. The cowboys shoot at each other in turns, as indicated by the variable $\codify{t}$, until one of them gets hit ($\codify{x}$ is set to $\codify{1}$). The variable $\codify{c}$ just counts the number of shots of the first cowboy and $\codify{d}$ those of the second cowboy.%
%
\program{dueling_cowboys}{Dueling Cowboys}{t}

With \cref{prop:syntactic} and \cref{thm:rat_func_semantics} we can almost immediately conclude that \Pref{prog:dueling_cowboys} has a rational PGF on any input. The equation system $(EQS)$ defined above is
	\begin{align*}
		\begin{pmatrix}
		\sem{W}(X^0T^0) \\
		\sem{W}(X^0T^1)
		\end{pmatrix}
		\eeq
		\begin{pmatrix}
			0 & (1-a)C \\
			(1-b)D & 0
		\end{pmatrix}
		\cdot
		\begin{pmatrix}
		\sem{W}(X^0T^0) \\
		\sem{W}(X^0T^1)
		\end{pmatrix}
		\pplus
		\begin{pmatrix}
			aCX\\
			bDXT
		\end{pmatrix}
		~.
	\end{align*}
	This system has a unique solution for all $a, b \in [0,1]$.
	Solving yields the PGF
	\begin{align*}
		G \ccoloneqq \sem{W}(X^0T^0) \eeq \frac{aCX + (1-a)bCDTX}{1-(1-b)(1-a)CD}~.
	\end{align*}
	In this example, there is no need to apply the additional restriction \eqref{eq:restric} from \cref{thm:rat_func_semantics}.
	From $G$ we can easily read off the following statistics: The probability that the first cowboy wins ($\codify{x = 1}$ and $\codify{t = 0}$) equals $\frac{a}{1 - (1-a)(1-b)}$, and the expected total number of shots of the first cowboy is
	$
		\tfrac{\partial}{\partial C} G(\vec{1}) = \frac{1}{a + b - a b}.
	$
	Notice that this quantity equals $\infty$ if $a$ and $b$ are both zero, i.e.\ if both cowboys have zero hit rate.
	Moreover, we can prove that $C$ and $D$ (as random variables) are not independent: It suffices to check that $G_C \cdot G_D \neq G_{C,D}$, where $G_\bvec{V}$ is the PGF obtained by substituting all variables not in $\bvec{V}$ with $1$. We emphasize that all calculations in this example could be easily carried out with a computer algebra system.\hfill$\triangle$
\end{example}
